Learning Variational Data Assimilation Models and Solvers

This paper addresses variational data assimilation from a learning point of view. Data assimilation aims to reconstruct the time evolution of some state given a series of observations, possibly noisy and irregularly-sampled. Using automatic differentiation tools embedded in deep learning frameworks, we introduce end-to-end neural network architectures for data assimilation. It comprises two key components: a variational model and a gradient-based solver both implemented as neural networks. A key feature of the proposed end-to-end learning architecture is that we may train the NN models using both supervised and unsupervised strategies. Our numerical experiments on Lorenz-63 and Lorenz-96 systems report significant gain w.r.t. a classic gradient-based minimization of the variational cost both in terms of reconstruction performance and optimization complexity. Intriguingly, we also show that the variational models issued from the true Lorenz-63 and Lorenz-96 ODE representations may not lead to the best reconstruction performance. We believe these results may open new research avenues for the specification of assimilation models in geoscience.

==> learning4DVar (3)/makefile <==
# Liste des .pdf du projet
PDF = preprint4DVarNN.pdf

# Commande de compilation
LATEX = pdflatex -interaction=batchmode
BIBTEX = bibtex -terse

#BIBTEX = bibtex
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
UNDEFINED = "((Reference|Citation).*undefined)|(Label.*multiply defined)"
	#Dépendance pour les .pdf
TEX=$(PDF: .pdf = .tex)

#
#	Commande de compilation
#
pdffiles: $(PDF)

# Commande de compilation
%.pdf : %.tex
	@echo "Compilation du tex"
	@$(LATEX) $<
	#@makeindex $*
	@# Etape de compilation suivant la nécessité.
	@if egrep -q $(RERUN) $*.log ; then echo "passe BibTex/LaTeX" ;\
	$(BIBTEX) $* ; $(LATEX) $<;  fi
	@if egrep -q $(RERUN) $*.log ; then echo "passe BibTex/LaTeX" ;\
	$(BIBTEX) $* ; $(LATEX) $<;  fi
	@if egrep -q $(UNDEFINED) $*.log ; then echo "passe Complémentaire";\
	$(BIBTEX) $* ; $(LATEX) $<;  fi
	@# Vérification de la présence de toute la biblio.
	@egrep -i $(UNDEFINED) $*.log || echo "Dépendance biblio non manquante"
	@exit 0


clean:
	rm -f *.dvi *.ps *.log *.aux *.out  *.idx *.toc *.blg *.bbl \
		*.ind *.ilg *.nav *.snm
	#rm -f *_database.bib *_database.bib.bak
	rm -f `find | grep .*~`

#
#  Construct difference file and prepare compilation for editting
#
FILE = preprint4DVarNN.tex
#FIGURES = 
DIFF_DIR = ./diff/
VERSION_OF_REFERENCE = ./version/$(FILE)

paper_diff:
	# 1. Create directory for diff.
	mkdir -p $(DIFF_DIR)
	# 2. Copy local files for the compilation
	cp ./makefile ./arxiv.sty ./zotero.bib $(DIFF_DIR)
	#cp -rf ./figures/ $(DIFF_DIR)
	# 3. Don't load figures for export.
	#./set_demo ./header-private.sty $(DIFF_DIR)header-private.sty
	# 4. Create the `diff file` 
	latexdiff $(VERSION_OF_REFERENCE) ./$(FILE) > $(DIFF_DIR)$(FILE)
	


==> makefile <==
# Liste des .pdf du projet
PDF = preprint4DVarNN.pdf

# Commande de compilation
LATEX = pdflatex -interaction=batchmode
BIBTEX = bibtex -terse

#BIBTEX = bibtex
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
UNDEFINED = "((Reference|Citation).*undefined)|(Label.*multiply defined)"
	#Dépendance pour les .pdf
TEX=$(PDF: .pdf = .tex)

#
#	Commande de compilation
#
pdffiles: $(PDF)

# Commande de compilation
%.pdf : %.tex
	@echo "Compilation du tex"
	@$(LATEX) $<
	#@makeindex $*
	@# Etape de compilation suivant la nécessité.
	@if egrep -q $(RERUN) $*.log ; then echo "passe BibTex/LaTeX" ;\
	$(BIBTEX) $* ; $(LATEX) $<;  fi
	@if egrep -q $(RERUN) $*.log ; then echo "passe BibTex/LaTeX" ;\
	$(BIBTEX) $* ; $(LATEX) $<;  fi
	@if egrep -q $(UNDEFINED) $*.log ; then echo "passe Complémentaire";\
	$(BIBTEX) $* ; $(LATEX) $<;  fi
	@# Vérification de la présence de toute la biblio.
	@egrep -i $(UNDEFINED) $*.log || echo "Dépendance biblio non manquante"
	@exit 0


clean:
	rm -f *.dvi *.ps *.log *.aux *.out  *.idx *.toc *.blg *.bbl \
		*.ind *.ilg *.nav *.snm
	#rm -f *_database.bib *_database.bib.bak
	rm -f `find | grep .*~`

#
#  Construct difference file and prepare compilation for editting
#
FILE = preprint4DVarNN.tex
#FIGURES = 
DIFF_DIR = ./diff/
VERSION_OF_REFERENCE = ./version/$(FILE)

paper_diff:
	# 1. Create directory for diff.
	mkdir -p $(DIFF_DIR)
	# 2. Copy local files for the compilation
	cp ./makefile ./arxiv.sty ./zotero.bib $(DIFF_DIR)
	#cp -rf ./figures/ $(DIFF_DIR)
	# 3. Don't load figures for export.
	#./set_demo ./header-private.sty $(DIFF_DIR)header-private.sty
	# 4. Create the `diff file` 
	latexdiff $(VERSION_OF_REFERENCE) ./$(FILE) > $(DIFF_DIR)$(FILE)
	

